Best-of-Both-Worlds Algorithms for Linear Contextual Bandits

We study best-of-both-worlds algorithms for $K$-armed linear contextual bandits. Our algorithms deliver near-optimal regret bounds in both the adversarial and stochastic regimes, without prior knowledge about the environment. In the stochastic regime, we achieve the polylogarithmic rate $\frac{(dK)^2\mathrm{poly}\log(dKT)}{\Delta_{\min}}$, where $\Delta_{\min}$ is the minimum suboptimality gap over the $d$-dimensional context space. In the adversarial regime, we obtain either the first-order $\widetilde{O}(dK\sqrt{L^*})$ bound, or the second-order $\widetilde{O}(dK\sqrt{\Lambda^*})$ bound, where $L^*$ is the cumulative loss of the best action and $\Lambda^*$ is a notion of the cumulative second moment for the losses incurred by the algorithm. Moreover, we develop an algorithm based on FTRL with Shannon entropy regularizer that does not require the knowledge of the inverse of the covariance matrix, and achieves a polylogarithmic regret in the stochastic regime while obtaining $\widetilde{O}\big(dK\sqrt{T}\big)$ regret bounds in the adversarial regime.

==> experiments.tex <==
%\section{Experiments}\label{sec:experiments}


% \begin{figure}[t]
% \centering
% % \includegraphics[width=0.22\textwidth]{figure/sample_fig.pdf}
% % \includegraphics[width=0.22\textwidth]{figure/sample_fig.pdf}
% %\vspace{-3mm}
% \caption{Cumulative loss of \textsf{Proposed method} \& baselines (parameters).}\label{fig:experiment_main}
% \end{figure}



\begin{itemize}
    \item FTRL with Shannon entropy

    % \item Algorithms with reduction approach: Algorithm~\ref{alg:LSBtoBOBW}, \ref{alg:LSBviaCorral} and \ref{alg:real_linexp3} 
    
    % \item Algorithm~\ref{alg:LSBtoBOBW}, dd-LSB via Corral (Algorithm 6 \citep{Dann+2023}) and Algorithm \ref{alg:secondorder_linearcon} (we need to simplify the part of continuous exponential weights computation)
    \item Stochastic baseline
    \item RealLinEXP~\citep{neu2020efficient}

    % \item \citep{olkhovskaya2023first} (we need to simplify the part of continuous exponential weights computation) 
\end{itemize}
More experimental results and details of experimental settings are provided in \Cref{appendix:experiments}.




==> tables.tex <==

\begin{table*}[t]
	\centering
	\caption{ Existing Results for  Linear or combinatorial full-bandit. $\cA$ is an action space. In linear bandit,   $\cA \subset \mathbb{R}^d$, and in combinatorial bandit,   $\cA \subset \{0,1\}^d$. $L_{*}$ is the cumulative loss of the best action. $\nu \leq d$	 is the self-concordance parameter. $m$ is the maximum size of actions $m=\max_{a \in \cA}\|a\|$. In \citet{Tsuchiya+2023}, $k$ is the number of actions and $n$ is the number of outcomes, $b \leq k n$ is the maximum number of distinct observations per action. In \cite{LinTian2014}, %$B_{\Delta}=O\left( \right)$ 
  $\sigma \subseteq {\cA}$ is the global observable set and $\beta_{\sigma}$ is the upper bound of estimation error bound. } 
	\label{table:linear_results}
 \scalebox{0.7}{
	

 %\arraystretch{2.3}{
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Setting & Algorithm & Adversarial & Stochastic  &  Sto.+Corruption \\

        \hline
           
        Linear bandit & \cite{Lee+2021} & $\sqrt{dT \log (|\cA|T) \log T}$  & $\frac{d\log(|\cA|T)\log T}{\Delta}$  &\\
		\hline
  
        Linear bandit & (Col.12)~\cite{Dann+2023} & $O(\sqrt{dT \log |\cX|})$ & $O(\frac{d \log |\cX| \log T}{\Delta}$)   &  $R^{\mathrm{sto}}_T+\sqrt{R^{\mathrm{sto}}_T \cdot C}$ \\
		\hline
        
        Partial (local obs.) & \cite{Tsuchiya+2023}  & $O(bk^{\frac{2}{3}} \sqrt{T \log T \log k_{\Pi}} )$  & $\frac{b^2k^4 \log T \log (k_{\pi}T)}{\Delta}$  &$R^{\mathrm{sto}}_T+\sqrt{R^{\mathrm{sto}}_T \cdot C}$\\
		\hline
  
        Partial (glocal obs.) & \cite{Tsuchiya+2023}  & $O((c_{\cG}T)^{\frac{2}{3}} (\log T \log(k_{\Pi}T)^{1/3})  $  & $\frac{c_{\cG}^2 \log T \log (k_{\Pi}T)}{\Delta^2}$  &$R^{\mathrm{sto}}_T+(R^{\mathrm{sto}}_T \cdot C^2)^{1/3}$\\
		\hline  

        Combinatorial full-bandit & \cite{cesa2012combinatorial}  & $O(\sqrt{  (1+\frac{2m^2}{d\lambda_{\min} })   d T \log|\cA| }$ && \\
		\hline  
  
        Combinatorial full-bandit & \cite{combes2015combinatorial}  & $O(\sqrt{ m^3 d T (1+\frac{m^{1/2}}{d \lambda_{\min}})} ) $ && \\
		\hline  

        Com. $\cX=\{0,1\}^d$ &  \citet{Zimmert+19} & $O(d\sqrt{T} ) $ & $O(\sum_{i: \Delta_i \neq 0}  \frac{\log T}{\Delta_i})$  & \\
		\hline  
  
  %       size-$m$ nonlinear obs. &  \citet{Agarwal+2021} &  & $O(m^\frac{1}{2}d^{\frac{1}{3}}T^{\frac{2}{3}}) $ & \\
		% \hline  
        size-$m$ full-bandit &  \citet{Idan2019} &  & $\frac{d m \log T}{\Delta}$  & \\
		\hline  

        Combinatorial Partial-linear &  \citet{LinTian2014} &  & $O(\sum_{x \in \sigma} \frac{\Delta_x \beta_{\sigma}^2 \log (T |\cA|) }{\Delta^2}+ 
  \frac{\Delta_{\max}\beta_{\sigma}^3}{\Delta_{\min}^3})$  & \\
		\hline   
  
         Combinatorial Partial-linear &  
          \citet{ChaudhuriT16} &  & $O(\sum_{x \in \sigma} \frac{\Delta_x \beta_{\sigma}^2 \log (T |\cA|) }{\Delta^2}+\frac{\beta^2_{\sigma}}{\Delta} \log \frac{\beta^2_{\sigma}}{\Delta} )$  & \\
		\hline   
  
         Combinatorial full-bandit &  \textbf{Algorithm~ \ref{alg:LSBtoBOBW}, \ref{alg:LSBviaCorral} and \ref{alg:comband}}& $\tilde{O}\left( \max\left\{d, \frac{m^2}{\lambda_{\min}}\right\} \sqrt{T \ln |A|}\right)$  & $O\left(\frac{\max\{d^2, \frac{m^4}{\lambda^2_{\min}}\}\ln |A| \log T}{\Delta} \right)$   &$R^{\mathrm{sto}}_T+\sqrt{R^{\mathrm{sto}}_T \cdot C}$\\
		\hline    
        \end{tabular}

        }
 %}
	
\end{table*}




\begin{table*}[t]
	\centering
	\caption{Contextual Bandit
	} 
	\label{table:adversarialresults}
 \scalebox{0.75}{
	

 %\arraystretch{0.5}{
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		Setting & Work &  Adversarial & Stochastic & Sto.+Corruption\\

            \hline
  
        Expert advice & (Col.13)~\cite{Dann+2023} & $O(\sqrt{K \log |\Pi|T })$ & $O(\frac{K \log |\Pi| \log T}{\Delta}$)     &$R^{\mathrm{sto}}_T+\sqrt{R^{\mathrm{sto}}_T \cdot C}$ \\
		\hline
  
 $X_t \sim \cD,\cA =[K]$  & \cite{neu2020efficient}(REALLINEXP3) &  $\tilde{O}(\sqrt{KdT})$  &    & \\
		\hline
 $X_t \sim \cD,\cA =[K]$, misspecified & \cite{neu2020efficient}(ROBUSTLINEXP3) &    $\tilde{O}((Kd)^{1/3}T^{2/3})$ &    & \\
		\hline


     $X_t \sim \cD$, $\cA \subseteq \{0,1\}^K$ & \cite{Zierahn+2023} & $\tilde{O}(mKT(a+\ln \frac{K}{m})\max\{d, \frac{m \sigma^2 \ln T}{\lambda_{\min}(\Sigma)} \} )$  &    & \\
     \hline
     $\SigmaInv$ is given(?) & \cite{He+2o22} &    &  $\tilde{O}(d\sqrt{T})$   & $\tilde{O}(d\sqrt{T})$ \\

		\hline
  
  %  $X_t \sim \cD$+BOTW  & Open &   &    & \\
		% \hline
  
  
 % model selection & \cite{pacchiano2022best}(ROBUSTLINEXP3) &    $\tilde{O}((Kd)^{1/3}T^{2/3})$ &    & \\
	% 	\hline		        
            
            
        \end{tabular}
        }
 %}
	
\end{table*}







\begin{table*}[t]
	\centering
	\caption{ Some Existing Results for  Stochastic/Adversarial  Combinatorial/Linear bandit
	} 
	\label{table:acversarialresults}
 \scalebox{0.7}{
	

 %\arraystretch{0.5}{
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Work & World & Loss & Feedback &Action Space\\

            \hline
            \citep{Bubeck+2012,WeiLuo2018, dani2008price} & Adv. & Linear & Linear  &$\cX \subset \mathbf{R}^d $ \\
		\hline
            % \citet{WeiLuo2018} & Adv. & Linear & Linear  &$\cX \subset \mathbf{R}^d $ \\
            % \hline
            	   \citet{Bogunovic+2020} & Sto. with Adv. Corruption &  Linear & Linear &$\cX \subset \mathbf{R}^d $ \\
		\hline
			  \citet{Lee+2021}  & Three worlds & Linear & Linear  &$\cX \subset \mathbf{R}^d $ \\
		\hline
		   \citet{Ito2021,Zimmert+19} & Three worlds &  Linear & Semi-bandit  &$\cX \subset \{0,1\}^d $\\
            \hline
		   % \citet{Zimmert+19} & Three worlds &  Linear & Semi-bandit   &$\cX \subset \{0,1\}^d $ \\
     %        \hline
            \citet{Zimmert+19} & Sto. / Adv.  &  Linear & Full-bandit &$\cX = \{0,1\}^d $ \\
            \hline
            \citet{XuLi2021} & Sto. with Adv. Corruption &  Linear & Semi-bandit   &$\cX \subset \{0,1\}^d $, Exact Oracle\\
            \hline
            \citet{Ito2022} & Three worlds &  Submodular (min) &  Bandit ($f_t(X_t)$)   &$2^{[n]}$, Exact Oracle\\
            \hline
            \citet{Harvey+2020} & Adv. &  Submodular (max) &  Full-information   &$2^{[n]}$, Approximate-regret\\
            \hline 
            
           Open & Adv./Sto. with Adv. Corruption  & Linear &  Full-Bandit  &$\cX \subset \{0,1\}^d $\\
            \hline           
            
            
        \end{tabular}
        }
 %}
	
\end{table*}



